Conditioning in Probabilistic Programming

We investigate the semantic intricacies of conditioning, a main feature in probabilistic programming. We provide a weakest (liberal) pre-condition (w(l)p) semantics for the elementary probabilistic programming language pGCL extended with conditioning. We prove that quantitative weakest (liberal) pre-conditions coincide with conditional (liberal) expected rewards in Markov chains and show that semantically conditioning is a truly conservative extension. We present two program transformations which entirely eliminate conditioning from any program and prove their correctness using the w(l)p-semantics. Finally, we show how the w(l)p-semantics can be used to determine conditional probabilities in a parametric anonymity protocol and show that an inductive w(l)p-semantics for conditioning in non-deterministic probabilistic programs cannot exist.

==> alt_nondet.tex <==
% !TEX root = main.tex
%\subsection{Non--Existence of \cwp for non-deterministic choice}
In~\cite{DBLP:journals/pe/GretzKM14} they state that positional\footnote{Also called memoryless.} schedulers suffice to implement demonic choice in an RMDP.
Accordingly, the expectation transformers \wp and \wlp resolve the choice $\NDChoice{P}{Q}$ between two programs $P$ and $Q$ by taking the pointwise minimum, \cf Figure~\ref{fig:cwp}.
This means that in a program location that offers a non-deterministic choice a decision can be made by evaluating the expectations using the current variable valuation $\sigma$ in that location.
%Thus subprogram $P$ is chosen if $\wp[P](f)(\sigma) \leq \wp[Q](f)(\sigma)$ and otherwise $Q$ is chosen.

In the following we illustrate why positional schedulers are not sufficient to determine the conditional expected reward in an RMDP.
This is closely related to a result due to~\cite{DBLP:conf/tacas/AndresR08}.
As a consequence we do not have a \cwp rule for non-deterministic choice that tells us how to compute the minimal conditional expectation from the current valuation and the \cwp[P] and \cwp[Q] of the two subprograms $P$ and $Q$.

Consider the RMDP \rmdp\ in Figure~\ref{fig:rmdp-counterexample}.
\begin{figure}
    \input{pics/alt_nondetproof}
	\caption{Positional schedulers do not suffice in this RMDP.}
    \label{fig:rmdp-counterexample}
\end{figure}
There are only two schedulers. Let $\sched_l$ be the scheduler that chooses to go from $P_5$ to $P_2$ and let $\sched_r$ be the scheduler that chooses $P_4$ as the successor of $P_5$.
Finally let $T=\{P_1, P_2, P_3\}$ and $U=\{\bad\}$.
Then we calculate $\CExpRew {\presuper{\sched_{l}}{\rdtmc}} {\Finally T} {\neg\Finally U} = 1.5$ and $\CExpRew {\presuper{\sched_{r}}{\rdtmc}} {\Finally T} {\neg\Finally U} = 1.4$.
Hence $\CExpRew \rmdp {\Finally T} {\neg\Finally U} = 1.4$ and the minimising scheduler is $\sched_r$.
However if we only consider the subsystem \rmdp' that starts execution in state $P_5$ we obtain $\CExpRew {\presuper{\sched_{l}}{\rdtmc'}} {\Finally T} {\neg\Finally U} = 2$ and $\CExpRew {\presuper{\sched_{r}}{\rdtmc'}} {\Finally T} {\neg\Finally U} = 2.2$.
So in that subsystem the minimising choice is given by $\sched_l$.
This shows how choices are resolved depending on the ``context'' within which the state occurs in the system.
As mentioned above~\cite{DBLP:conf/tacas/AndresR08} show that a particular class of history dependent schedulers is needed to find the conditional expected reward.

This example shows that any attempt to define a \cwp transformer for non-deterministic choice as 
\[\cwp[\NDChoice{P}{Q}](X) \eqdef \lambda \sigma \mydot\min_{\preccurlyeq}\{\cwp[P](X)(\sigma),\wp[Q](X)(\sigma)\}\]
must fail for any representation of conditional expectations $X$ and any order $\preccurlyeq$ between them because the decision is made at a point where the ``context'' information is missing.
In this sense no inductive definition of a conditional expectation transformer is possible.

To remedy this one could think of a transformer that does not resolve choices immediately but delays the decision between subprograms until the whole program has been evaluated.
We would call such a transformer a \emph{powerset expectation transformer} because it must keep track of all possible combinations of decisions.
However it seems that this straightforward approach is impractical, particularly in the context of loops.
At this stage the conditional expectation transformer semantics for non-deterministic choice remain a problem for future work.

==> nondetapp.tex <==
\subsection{Proof of Theorem \ref{thm:nocpet}}
\label{proofof:thm:nocpet}

\begingroup
\def\thelemma{\ref{thm:nocpet}}
\begin{theorem}
There exists no inductive CPET.
\end{theorem}
\addtocounter{lemma}{-1}
\endgroup


\begin{proof}
The proof goes by contradiction.
Consider the program $P = \PChoice{P_1}{\nicefrac 1 2}{P_5}$ with 
\begin{align*}
P_1 ~&=~ \Ass x 1\\
P_5 ~&=~ \NDChoice{P_2}{P_4}\\
P_2 ~&=~ \Ass x 2\\
P_4 ~&=~ \PChoice{\Observe~\texttt{false}}{\nicefrac 1 2}{P_{2+\varepsilon}}\\
P_{2+\varepsilon} ~&=~ \Ass x {2 + \varepsilon}~,
\end{align*}
where $\varepsilon > 0$.
A schematic depiction of the RMDP $\Rmdp{\sigma}{x}{P}$ is given in Figure~\ref{fig:rmdpschem}.
\begin{figure}
	\centering
    \input{pics/nondetproof}
    \caption{Schematic depiction of the RMDP $\Rmdp{\sigma}{x}{P}$}
    \label{fig:rmdpschem}
\end{figure}
Assume there exists an inductive CPET $\cwp^*$ over some appropriate domain $D$. Then,
\begin{align*}
\cwp^*[P_1] ~&=~ x_1, \text{ with } \llbracket x_1 \rrbracket = 1\\
\cwp^*[P_2] ~&=~ x_2, \text{ with } \llbracket x_2 \rrbracket = 2\\
\cwp^*[P_{2 + \varepsilon}] ~&=~ x_{2 + \varepsilon}, \text{ with } \llbracket x_{2 + \varepsilon} \rrbracket = {2 + \varepsilon}\\
\cwp^*[\texttt{observe false}] ~&=~ \mathfrak{of}, \text{ with } \llbracket \mathfrak{of} \rrbracket = \bot
\end{align*}
for some appropriate $x_1,\, x_2 ,\, x_{2 + \varepsilon},\, \mathfrak{of} \in D$.
By Definition \ref{def:inductiveCPETs}, $\cwp^*$ being inductive requires the existence of a function $\mathcal P$, such that
\begin{align*}
\cwp^*[P_4] ~=~ &\mathcal{K}\left(\cwp^*[\Observe~\texttt{false}],\, \nicefrac{1}{2},\, \cwp^*[P_{2+\varepsilon}]\right)\\
~=~ &\mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})~.
\end{align*}
In addition, there must be an $\mathcal N$ with:
\begin{align*}
\cwp^*[P_5] ~=~ &\mathcal{N}\left(\cwp^*[P_2],\, \cwp^*[P_4]\right)\\
~=~ &\mathcal N (x_2,\, \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon}))~.
\end{align*}
Since $P_4$ is a probabilistic choice between an infeasible branch and $P_{2 + \varepsilon}$, the expected value for $x$ has to be rescaled to the feasible branch. 
Hence $P_4$ yields $\llbracket \cwp^*[P_4] \rrbracket = 2 + \varepsilon$, whereas $\llbracket \cwp^*[P_2] \rrbracket = 2$. 
Thus:
\begin{align}
\llbracket x_2 \rrbracket ~\lneq~ \llbracket \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})\rrbracket \label{x2neqprob}
\end{align}
As non--deterministic choice is demonic, we have:
\begin{align}
\cwp^*[P_5] ~=~ \mathcal N (x_2,\, \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})) ~=~ x_{2}\label{P4eqx2}
\end{align}
As $\mathcal{N}\left(\cwp^*[P_2],\, \cwp^*[P_4]\right) \in \{\cwp^*[P_2],\, \cwp^*[P_4]\}$ we can resolve non--determinism in $P$ by either rewriting $P$ to $\PChoice{P_1}{\nicefrac 1 2}{P_2}$ which gives 
\begin{align*}
\llbracket \cwp^*\PChoice{P_1}{\nicefrac 1 2}{P_2} \rrbracket ~=~ &\frac{3}{2}~,
\intertext{or we rewrite $P$ to $\PChoice{P_1}{\nicefrac 1 2}{P_4}$, which gives}
\llbracket \cwp^*\PChoice{P_1}{\nicefrac 1 2}{P_4} \rrbracket ~=~ &\frac{4 + \varepsilon}{3}~.
\end{align*} 
For a sufficiently small $\varepsilon$ the second option should be preferred by a demonic scheduler. 
This, however, suggests:
\begin{align*}
\cwp^*[P_5] ~=~ &\mathcal N (x_2,\, \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon}))\\
=~ &\mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})
\end{align*}
Together with Equality (\ref{P4eqx2}) we get $x_2 = \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})$, which implies $\llbracket x_2 \rrbracket = \llbracket \mathcal{K}(\mathfrak{of},\, \nicefrac 1 2,\, x_{2 + \varepsilon})\rrbracket$.
This is a contradiction to Inequality (\ref{x2neqprob}).
\end{proof}




%\subsection{Proof of Corollary \ref{cor:cwpnondet}}
%\label{proofof:cor:cwpnondet}
%
%\begingroup
%\def\thecorollary{\ref{cor:cwpnondet}}
%\begin{corollary}
%We cannot extend the \cwp rules in Figure \ref{fig:cwp} for non--deterministic programs such that Theorem \ref{thm:correspondence:cwp} extends to full \cpGCL.
%\end{corollary}
%\addtocounter{corollary}{-1}
%\endgroup
%
%
%\begin{proof}
%We first show how we can define an inductive CPET for $\cpGCL^{-}$ by means of $\cwp$.
%As the domain we take $D = \Ex \times \BEx$ and for the interpretation function we set $\llbracket (f,\, g) \rrbracket. For the probabilistic choice we have
%\end{proof}

==> pldimacros.tex <==
\newcommand{\pGCL}{{\sc pGCL}\xspace}
% pGCL commands
\newcommand{\OBSERVE}{{\sf observe}\xspace}

% Numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Iint}{\{0,1\}\subseteq\mathbb{Z}} % integer interval 0,1
\newcommand{\Ireal}{[0,1]\subseteq\mathbb{R}}  % real interval [0,1]
\newcommand{\Irat}{[0,1]\subseteq\mathbb{Q}}  % real interval [0,1]
\newcommand{\Irealo}{(0,1]\subseteq\mathbb{R}} % open real interval (0,1]
\newcommand{\powerset}{\mathcal{P}}

% Comments
\newcommand{\nj}[1]{\todo[inline,color=black]{\color{yellow}NJ: #1}\color{black}}
\newcommand{\bk}[1]{\todo[inline,color=red!40]{BK: #1}}
\newcommand{\fo}[1]{\todo[inline,color=blue!40]{\color{black}FO: #1}\color{black}}
\newcommand{\fg}[1]{\todo[inline,color=green!40]{\color{black}FG: #1}\color{black}}
\newcommand{\jk}[1]{\todo[inline,color=orange]{\color{white}JPK: #1}\color{black}}

% Universes
\newcommand{\Pairs}{\mathbb{C}}
\newcommand{\Rpos}{\R_{{}\geq 0}}
\newcommand{\Rposinf}{\Rpos^{\infty}}
\newcommand{\Rposinfbot}{\Rpos^{\infty,\bot}}
\newcommand{\boundR}{\R_{[0,\, 1]}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\boundE}{\E_{{}\leq1}}
\newcommand{\States}{\mathbb{S}}
\newcommand{\Universe}{\mathcal{U}}

% Relations
\newcommand{\eq}{\sim}

% Operators
\newcommand{\Polter}[2]{\,\polter{\,#1\,}{\,#2\,}\,}

% Functions
\newcommand{\cwpf}{\textnormal{\textsf{cwp}}}
\newcommand{\cwpsharpf}{\textnormal{\textsf{cwp}}^\sharp}
\newcommand{\cwp}[2]{\cwpf[#1]#2}
\newcommand{\cwpsharp}[2]{\cwpsharpf[#1]#2}



==> semantics.tex <==

\section{Semantics}

\subsection{Denotational}

\begin{Definition}[Expectations]
An \emph{expectation} is a function $f\colon \States \rightarrow \Rposinf$. 
We denote the set of all expectations by $\E$.
A \emph{bounded expectation} is a function $g\colon \States \rightarrow \mathbb{R}_{[0,\, 1]}$. 
We denote the set of all bounded expectations by $\boundE$.
\end{Definition}

\begin{Definition}[Conditional Expectations]
A pair $(f,\, g) \in \E \times \boundE$ is called a \emph{conditional expectation}.
We denote the set of all conditional expectations by $\Pairs$.
\end{Definition}

\begin{Definition}[Equivalence of Expectations]
Two conditional expectations $(f,\, g)$ and $(f',\, g')$ are \emph{equivalent}, denoted $(f,\, g) \eq (f',\, g')$ iff
\begin{align*}
\exists \, r > 0 ~~ \forall\, \sigma \colon &\big( f(\sigma) = r \cdot f'(\sigma) \,\wedge\, g(\sigma) = r \cdot g'(\sigma) \big)\\
& \,\vee\, \big( g(\sigma) = 0 \,\wedge\, g'(\sigma) = 0\big)~.
\end{align*}
\end{Definition}

\begin{Lemma}
$\eq$ is an equivalence relation on $\Pairs$.
\end{Lemma}

\begin{Definition}[Quotient of $\Pairs$ under $\eq$]
The quotient $\Pairs / {\eq}$ of $\Pairs$ under the equivalence relation $\eq$  is denoted by $\Universe$.
We denote an equivalence class by taking a representative, i.e.\ we denote
\begin{align*}
[f,\, g] ~:=~ \big\{(f',\, g') ~\big\vert~ (f',\, g') \eq (f, g)\big\} ~\in~ \Universe
\end{align*}•
\end{Definition}


\begin{Definition}[Ordering of $\Pairs$]
We define ${\sqsubseteq} \subseteq \Universe \times \Universe$ as follows:
\begin{align*}
[f,\, g] \sqsubseteq [f',\, g'] ~~\textnormal{ iff }~~ \forall\,\sigma\colon \Polter{f(\sigma)}{g(\sigma)} \leq \Polter{f'(\sigma)}{g'(\sigma)}
\end{align*}
\end{Definition}

\begin{Lemma}
$\sqsubseteq$ is a complete partial order on $\Universe$.
\end{Lemma}

\begin{Lemma}
$\cwpsharpf$ is independent of the representative with respect to $\sim$, i.e.\ 
\begin{align*}
(f,\, g) \sim (f',\, g') ~\implies~ \cwpsharp{P}{(f,\, g)} \sim \cwpsharp{P}{(f',\, g')}
\end{align*}•
\end{Lemma}






\paragraph{Generalisation of wp}
\paragraph{Program transformation that removes conditioning}

\subsection{Operational}

\subsection{Correspondence theorem}


==> todo.tex <==
%\vspace{5mm}
%
%\fbox{\parbox{\columnwidth}{
%MISSMATCHS TO UNIFY
%\begin{itemize}
%  \item ``expectation--transformer'' vs ``expctation transformer'' 
%  \item   ``$\Observe~G$'' vs ``$\Observe~(G)$''
%  \item  ``fully'' vs ``purely''
%  \item    program syntax: use or not a ``;'' in the final statement of a program
%  \item    ``if-then-else'' vs ``ite''
%   \item    ``:'' vs ``;'' at the end of theorem statement, before formulae.
%   \item ``--'' vs ``---''
%   \item  ``operator'' vs ``transformer'' 
%\end{itemize}
%
%TODO
%\begin{itemize}
%\item Change ``-'' to ``--''  in compound words. 
%\end{itemize}
%
%}}
